Realistic Full-Body Anonymization with Surface-Guided GANs

Recent work on image anonymization has shown that generative adversarial networks (GANs) can generate near-photorealistic faces to anonymize individuals. However, scaling up these networks to the entire human body has remained a challenging and yet unsolved task. We propose a new anonymization method that generates realistic humans for in-the-wild images. A key part of our design is to guide adversarial nets by dense pixel-to-surface correspondences between an image and a canonical 3D surface. We introduce Variational Surface-Adaptive Modulation (V-SAM) that embeds surface information throughout the generator. Combining this with our novel discriminator surface supervision loss, the generator can synthesize high quality humans with diverse appearances in complex and varying scenes. We demonstrate that surface guidance significantly improves image quality and diversity of samples, yielding a highly practical generator. Finally, we show that our method preserves data usability without infringing privacy when collecting image datasets for training computer vision models. Source code and appendix is available at: \href{https://github.com/hukkelas/full_body_anonymization}{github.com/hukkelas/full\_body\_anonymization}

==> tex/experiments/coco_training_table.tex <==
\begin{table*}[t]
    \caption{
        Instance segmentation mask AP on the COCO validation set \cite{lin2014microsoft}.
        The results are from a Mask R-CNN \cite{he2017mask} \href{https://github.com/facebookresearch/detectron2/blob/335b19830e4ea5c5a74a085a04ff4a2f1a1dbf71/configs/COCO-InstanceSegmentation/mask_rcnn_R_50_FPN_3x.yaml}{R50-FPN-3x} from detectron2 \cite{wu2019detectron2} trained on different anonymized datasets.
        The validation set is not anonymized.
        }
    \label{tab:coco_training}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
        \hline
        \textbf{Training} Dataset & AP$_{50:95}$ $\uparrow$ & AP$_{50}$ $\uparrow$ & AP$_{75}$ $\uparrow$ & AP$_{\text{s}}$ $\uparrow$ & AP$_{\text{m}}$ $\uparrow$& AP$_{\text{l}}$ $\uparrow$ & AP$_\text{Person}$ $\uparrow$ \\
        \hline
        \hline
        Original                       & 37.1                           & 58.7                           & 39.8                           & 18.8                           & 39.6                           & 53.3                           & 47.8                           \\
        \hline
        \hline
        Mask Out                       & 34.6                           & 55.2                           & 36.7                           & 16.7                           & 36.5                           & 50.0                           & 44.7                           \\
        \hline
        $8 \times 8$ Pixelation        & 34.8                           & 55.7                           & 37.0                           & 16.9                           & \textbf{36.7}                           & 50.3                           & 46.5                           \\
        \hline
        $16 \times 16$ Pixelation      & \textbf{35.0}                           & 55.9                           & 37.3                           & 17.3                           & 37.1                           & 50.4                           & \textbf{46.9}                           \\
        \hline
        Ours                           & \textbf{35.0}                           & \textbf{56.0}                           & \textbf{37.5}                           & \textbf{17.7}                           & \textbf{36.7}                           & \textbf{50.6}                           & 46.5                           \\
        \hline
    \end{tabular}
\end{table*}

==> tex/experiments/mapping_dimensionality.tex <==

\begin{table*}
    \caption{
        The effect of the dimensionality of $\omega_i$ on image quality.
        Note that we keep the complexity of $f_\omega$ constant through the experiments, and the sole change is the output dimensionality of $\omega_i$.
        Dimensionality of $\omega_i$ is equivalent to the number of neurons in the last fully-connected layer of $f_\omega$.
        \modulationMetodNoiseShort parameters includes $f_\omega$ and layer-wise affine transformation, where $\omega_i$ dimensionality primarily affects the latter.
        }
    \label{tab:mapping_dimensionality}
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|}
        \hline
        Dimensionality of $\omega_i$ & LPIPS $\downarrow$  & FID $\downarrow$ & PPL $\downarrow$ & LPIPS Diversity $\uparrow$ & Face FID $\downarrow$ & \modulationMetodNoiseShort Parameters \\
        \hline
        \hline
        32                             & 0.218                          & 4.7                            & 29.8                           & 0.171                          & 7.5                            & 3.0M\\
        \hline
        64                             & 0.219                          & 4.7                            & 27.5                           & 0.175                          & 7.3                            & 3.3M\\
        \hline
        128                            & 0.218                          & 4.6                            & 21.7                           & 0.176                          & 7.2                            & 3.9M \\
        \hline
        256                            & 0.218                          & 4.9                            & 19.9                           & 0.175                          & 8.1                            & 5.2M\\
        \hline
        512 (default)                  & 0.217                          & 4.5                            & 18.1                           & 0.173                          & 7.1                            & 7.8M\\
        \hline        
    \end{tabular}
\end{table*}


==> tex/experiments/pascal_training_table.tex <==
\begin{table}
    \caption{
        Object Detection AP on the PASCAL VOC validation set \cite{everingham10pascal}.
        The results are from a Faster R-CNN \cite{ren2015faster} \href{https://github.com/facebookresearch/detectron2/blob/335b19830e4ea5c5a74a085a04ff4a2f1a1dbf71/configs/PascalVOC-Detection/faster_rcnn_R_50_C4.yaml}{R50-C4} from detectron2 \cite{wu2019detectron2} trained on different anonymized datasets.
        The validation set is not anonymized.
        }
    \label{tab:pascal_train}
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textbf{Training} Dataset & AP$_{50:95}$ $\uparrow$ & AP$_{50}$ $\uparrow$ & AP$_{75}$ $\uparrow$ \\
        \hline
        \hline
        Original                       & 51.8                           & 80.3                           & 56.5   \\
        \hline
        \hline
        Mask Out        & \textbf{51.3}                           & 80.0                           & 55.7   \\
        \hline
        $8 \times 8$ Pixelation        & 51.2                           & 79.9                           & 55.03   \\
        \hline
        $16 \times 16$ Pixelation        & 51.2                           & 79.8                           & 55.7   \\
        \hline
        Ours        & \textbf{51.3}                           & \textbf{80.1}                           & \textbf{56.0}   \\
        \hline
    \end{tabular}
\end{table}

==> tex/experiments/pascal_validation_table.tex <==
\begin{table}
    \caption{
        Object Detection AP on the PASCAL VOC validation set \cite{everingham10pascal}.
        The results are from a \textbf{pre-trained} Faster R-CNN \cite{ren2015faster} \href{https://github.com/facebookresearch/detectron2/blob/335b19830e4ea5c5a74a085a04ff4a2f1a1dbf71/configs/PascalVOC-Detection/faster_rcnn_R_50_C4.yaml}{R50-C4} from detectron2 \cite{wu2019detectron2}.
        }
    \label{tab:pascal_val}
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textbf{Validation} Dataset & AP$_{50:95}$ $\uparrow$ & AP$_{50}$ $\uparrow$ & AP$_{75}$ $\uparrow$ \\
        \hline
        \hline
        Original                       & 51.8                           & 80.3                           & 56.5   \\
        \hline
        \hline
        Mask Out        & 47.9                           & 75.2                           & 51.4   \\ 
        \hline
        $8 \times 8$ Pixelation        & 47.2                           & 75.1                           & 50.8   \\
        \hline
        $16 \times 16$ Pixelation        & 48.5                           & 76.7                           & 52.0   \\
        \hline
        Ours        & \textbf{50.3}                           & \textbf{78.9}                           & \textbf{54.2}   \\
        \hline
    \end{tabular}
    \end{adjustbox}
\end{table}

==> tex/experiments/semantic_modulation.tex <==
\begin{table}[t]
    \centering
    \caption{
        Comparison of \modulationMetodNoiseShort to semantic modulation methods.
        All modulation methods are applied on top of config B.}
    \label{tab:modulation_comparison}
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{|l|c|c|c|c|}
        \hline
        Method & LPIPS $\downarrow$ &  FID $\downarrow$ & PPL $\downarrow$ & Face FID $\downarrow$ \\
        \hline
        \hline
        CLADE \cite{Tan_2021CLADE}     & 0.224                          & 5.2                            & 24.1                           & 8.9                            \\
        \hline
        INADE \cite{tan2021INADE}      & 0.225                          & 5.4                            & 23.8                           & 9.4                            \\
        \hline
        SPADE \cite{Park_2019}         & 0.219                          & 5.0                            & 23.6                           & 8.7                            \\
        \hline
        \hline
        \modulationMetodShort          & 0.217                          & 4.8                            & 22.0                           & 7.8                            \\
        \hline
        \modulationMetodNoiseShort     & \textbf{0.217}                          & \textbf{4.5}                            & \textbf{18.1}                           & \textbf{7.1}                            \\
        \hline
    \end{tabular}
    \end{adjustbox}
\end{table}



==> tex/experiments/semantic_supervision.tex <==
\begin{table}[t]
    \centering
    \caption{
        Comparison of different generator conditioning methods in combination with semantic/surface discriminator supervision.
        *CSE/Semantic map is concatenated with input image.
        }
    \label{tab:semantic_comparison}
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{|l|l|c|c|c|c|}
        \hline
        Generator Conditioning & Supervision & Face FID $\downarrow$ & LPIPS Diversity  $\uparrow$ & FID $\downarrow$ & PPL $\downarrow$  \\
        \hline
        \hline
        Concatenate Semantic* & Semantic       & 10.9                         & 0.152                          & 7.4                            & 45.1                           \\
        \hline
        Concatenate CSE* & CSE                & 12.3                         & 0.157                          & 7.3                            & 40.4                           \\
        \hline
        \hline
        SPADE \cite{Park_2019} & Semantic                & 9.5                          & 0.142                          & 5.2                            & \textbf{14.0}                           \\
        \hline
        SPADE \cite{Park_2019} & CSE                    & 8.7                          & 0.164                          & 5.0                            & 23.6                           \\
        \hline
        \hline
        \modulationMetodNoiseShort & Semantic  & 10.2                         & 0.172                          & 6.0                            & 19.8                           \\
        \hline
        \modulationMetodNoiseShort & CSE & \textbf{7.1}                          & \textbf{0.173}                          & \textbf{4.5}                            & 18.1                           \\
        \hline
    \end{tabular}
    \end{adjustbox}
\end{table}

==> tex/figures/random_DF1.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/original/1243.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/1891.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/196.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/2060.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/2231.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/2304.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/2435.png}
\captionsetup{justification=centering,textfont=small}
\caption*{Original}
\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/1243.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/1891.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/196.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/2060.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/2231.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/2304.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/2435.png}
\captionsetup{justification=centering,textfont=small}
\caption*{Truncated $\omega$}
\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/1243.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/1891.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/196.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/2060.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/2231.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/2304.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/2435.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/1243.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/1891.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/196.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/2060.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/2231.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/2304.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/2435.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/1243.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/1891.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/196.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/2060.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/2231.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/2304.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/2435.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/1243.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/1891.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/196.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/2060.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/2231.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/2304.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/2435.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/1243.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/1891.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/196.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/2060.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/2231.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/2304.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/2435.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/1243.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/1891.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/196.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/2060.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/2231.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/2304.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/2435.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/1243.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/1891.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/196.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/2060.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/2231.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/2304.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/2435.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/1243.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/1891.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/196.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/2060.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/2231.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/2304.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/2435.png}
\end{subfigure}%%
\caption{
    Diverse synthesized images from DeepFashion-CSE.
    (b) shows generated results with a truncated latent, and all other columns use no truncation.
    Each column is synthesized with the same latent variable $z$.
    All images and latent variables are randomly sampled. Zoom in for details.
    }
\label{fig:random_DF1}
\end{figure*}

==> tex/figures/random_DF2.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/original/2625.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/4012.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/4459.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/4518.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/4871.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/6317.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/6936.png}
\captionsetup{justification=centering,textfont=small}
\caption*{Original}
\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/2625.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/4012.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/4459.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/4518.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/4871.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/6317.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/6936.png}
\captionsetup{justification=centering,textfont=small}
\caption*{Truncated $\omega$}
\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/2625.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/4012.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/4459.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/4518.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/4871.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/6317.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/6936.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/2625.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/4012.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/4459.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/4518.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/4871.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/6317.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/6936.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/2625.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/4012.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/4459.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/4518.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/4871.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/6317.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/6936.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/2625.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/4012.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/4459.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/4518.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/4871.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/6317.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/6936.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/2625.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/4012.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/4459.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/4518.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/4871.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/6317.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/6936.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/2625.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/4012.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/4459.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/4518.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/4871.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/6317.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/6936.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/2625.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/4012.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/4459.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/4518.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/4871.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/6317.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/6936.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/2625.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/4012.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/4459.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/4518.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/4871.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/6317.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/6936.png}

\end{subfigure}%%
\caption{
    Diverse synthesized images from DeepFashion-CSE.
    (b) shows generated results with a truncated latent, and all other columns use no truncation.
    Each column is synthesized with the same latent variable $z$.
    All images and latent variables are randomly sampled. Zoom in for details.
    }
\label{fig:random_DF2}
\end{figure*}

==> tex/figures/random_DF3.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/original/8173.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/838.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/881.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/8878.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/9470.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/original/9833.png}
\captionsetup{justification=centering,textfont=small}
\caption*{Original}
\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/8173.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/838.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/881.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/8878.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/9470.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_truncatedW/9833.png}
\captionsetup{justification=centering,textfont=small}
\caption*{Truncated $\omega$}
\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/8173.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/838.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/881.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/8878.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/9470.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z0/9833.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/8173.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/838.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/881.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/8878.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/9470.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z1/9833.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/8173.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/838.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/881.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/8878.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/9470.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z2/9833.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/8173.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/838.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/881.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/8878.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/9470.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z3/9833.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/8173.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/838.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/881.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/8878.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/9470.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z4/9833.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/8173.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/838.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/881.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/8878.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/9470.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z5/9833.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/8173.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/838.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/881.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/8878.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/9470.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z6/9833.png}

\end{subfigure}%%
\begin{subfigure}[t]{0.1\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/8173.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/838.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/881.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/8878.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/9470.png}
\includegraphics[width=\linewidth]{generated_images/random_DF/ours_z7/9833.png}

\end{subfigure}%%
\caption{
    Diverse synthesized images from DeepFashion-CSE.
    (b) shows generated results with a truncated latent, and all other columns use no truncation.
    Each column is synthesized with the same latent variable $z$.
    All images and latent variables are randomly sampled. Zoom in for details.
    }
\label{fig:random_DF3}
\end{figure*}

==> tex/figures/random_coco1.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000000785.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000046497.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000111609.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000144003.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000153011.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000164602.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000168337.jpg}
\caption*{Original}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000000785.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000046497.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000111609.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000144003.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000153011.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000164602.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000168337.jpg}
\caption*{Mask Out}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000000785.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000046497.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000111609.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000144003.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000153011.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000164602.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000168337.jpg}
\caption*{Pixelation $8 \times 8$}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000000785.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000046497.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000111609.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000144003.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000153011.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000164602.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000168337.jpg}
\caption*{Pixelation $16 \times 16$}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000000785.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000046497.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000111609.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000144003.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000153011.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000164602.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000168337.jpg}
\caption*{Ours}
\end{subfigure}%%
\caption{
    Randomly sampled images from the anonymized COCO \cite{lin2014microsoft} validation dataset.
    Each image is sampled with latent truncation (t=0), see \appendixQuantitative for details.
    Zoom in for details.
    } 
\label{fig:coco_random1}
\end{figure*}

==> tex/figures/random_coco2.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000186449.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000222118.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000249786.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000259097.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000260470.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000273493.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000276024.jpg}
\caption*{Original}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000186449.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000222118.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000249786.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000259097.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000260470.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000273493.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000276024.jpg}
\caption*{Mask Out}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000186449.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000222118.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000249786.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000259097.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000260470.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000273493.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000276024.jpg}
\caption*{Pixelation $8 \times 8$}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000186449.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000222118.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000249786.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000259097.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000260470.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000273493.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000276024.jpg}
\caption*{Pixelation $16 \times 16$}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000186449.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000222118.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000249786.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000259097.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000260470.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000273493.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000276024.jpg}
\caption*{Ours}
\end{subfigure}%%
\caption{
    Randomly sampled images from the anonymized COCO \cite{lin2014microsoft} validation dataset.
    Each image is sampled with latent truncation (t=0), see \appendixQuantitative for details.
    Zoom in for details.
    } 
\label{fig:coco_random2}
\end{figure*}

==> tex/figures/random_coco3.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000282298.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000286660.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000291791.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000311928.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000319607.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000341196.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000342367.jpg}
\caption*{Original}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000282298.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000286660.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000291791.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000311928.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000319607.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000341196.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000342367.jpg}
\caption*{Mask Out}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000282298.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000286660.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000291791.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000311928.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000319607.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000341196.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000342367.jpg}
\caption*{Pixelation $8 \times 8$}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000282298.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000286660.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000291791.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000311928.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000319607.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000341196.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000342367.jpg}
\caption*{Pixelation $16 \times 16$}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000282298.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000286660.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000291791.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000311928.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000319607.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000341196.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000342367.jpg}
\caption*{Ours}
\end{subfigure}%%
\caption{
    Randomly sampled images from the anonymized COCO \cite{lin2014microsoft} validation dataset.
    Each image is sampled with latent truncation (t=0), see \appendixQuantitative for details.
    Zoom in for details.
    } 
\label{fig:coco_random3}
\end{figure*}

==> tex/figures/random_coco4.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000455157.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000459662.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000464144.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000465179.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000470952.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000476215.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000486104.jpg}
\caption*{Original}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000455157.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000459662.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000464144.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000465179.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000470952.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000476215.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000486104.jpg}
\caption*{Mask Out}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000455157.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000459662.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000464144.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000465179.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000470952.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000476215.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000486104.jpg}
\caption*{Pixelation $8 \times 8$}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000455157.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000459662.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000464144.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000465179.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000470952.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000476215.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000486104.jpg}

\caption*{Pixelation $16 \times 16$}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000455157.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000459662.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000464144.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000465179.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000470952.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000476215.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000486104.jpg}
\caption*{Ours}
\end{subfigure}%%
\caption*{}
\caption{
    Randomly sampled images from the anonymized COCO \cite{lin2014microsoft} validation dataset.
    Each image is sampled with latent truncation (t=0), see \appendixQuantitative for details.
    Zoom in for details.
    } 
\label{fig:coco_random4}
\end{figure*}

==> tex/figures/random_coco5.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/original/000000502229.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/original/000000504415.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/original/000000527750.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/original/000000529939.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/original/000000531707.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/original/000000535306.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/original/000000542776.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/original/000000563470.jpg}
\caption*{Original}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/maskout_rand/000000502229.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/maskout_rand/000000504415.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/maskout_rand/000000527750.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/maskout_rand/000000529939.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/maskout_rand/000000531707.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/maskout_rand/000000535306.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/maskout_rand/000000542776.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/maskout_rand/000000563470.jpg}
\caption*{Mask Out}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation8/000000502229.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation8/000000504415.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation8/000000527750.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation8/000000529939.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation8/000000531707.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation8/000000535306.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation8/000000542776.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation8/000000563470.jpg}
\caption*{Pixelation $8 \times 8$}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation16/000000502229.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation16/000000504415.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation16/000000527750.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation16/000000529939.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation16/000000531707.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation16/000000535306.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation16/000000542776.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/pixelation16/000000563470.jpg}
\caption*{Pixelation $16 \times 16$}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/n6_large_512/000000502229.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/n6_large_512/000000504415.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/n6_large_512/000000527750.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/n6_large_512/000000529939.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/n6_large_512/000000531707.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/n6_large_512/000000535306.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/n6_large_512/000000542776.jpg}
\includegraphics[height=0.122\textheight]{generated_images/coco_random_examples/n6_large_512/000000563470.jpg}
\caption*{Ours}
\end{subfigure}%%
\caption{
    Randomly sampled images from the anonymized COCO \cite{lin2014microsoft} validation dataset.
    Each image is sampled with latent truncation (t=0), see \appendixQuantitative for details.
    Zoom in for details.
    } 
\label{fig:coco_random5}
\end{figure*}

==> tex/figures/random_coco6.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000345361.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000183716.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000276285.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/original/000000500565.jpg}
\caption*{Original}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000345361.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000183716.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000276285.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/maskout_rand/000000500565.jpg}
\caption*{Mask Out}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000345361.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000183716.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000276285.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation8/000000500565.jpg}
\caption*{Pixelation $8 \times 8$}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000345361.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000183716.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000276285.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/pixelation16/000000500565.jpg}
\caption*{Pixelation $16 \times 16$}
\end{subfigure}%%
\begin{subfigure}[t]{0.2\linewidth}
\centering
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000345361.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000183716.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000276285.jpg}
\includegraphics[height=0.120\textheight]{generated_images/coco_random_examples/n6_large_512/000000500565.jpg}
\caption*{Ours}
\end{subfigure}%%
\caption{
    Randomly sampled images from the anonymized COCO \cite{lin2014microsoft} validation dataset.
    Each image is sampled with latent truncation (t=0), see \appendixQuantitative for details.
    Zoom in for details.
    } 
\label{fig:coco_random6}
\end{figure*}

==> tex/figures/random_cse1.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/original/1028.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/1042.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/1123.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/1457.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/1599.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Original}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/1028.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/1042.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/1123.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/1457.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/1599.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{SPADE \cite{Park_2019}}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/1028.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/1042.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/1123.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/1457.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/1599.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config D}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/1028.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/1042.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/1123.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/1457.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/1599.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/1028.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/1042.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/1123.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/1457.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/1599.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/1028.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/1042.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/1123.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/1457.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/1599.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/1028.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/1042.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/1123.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/1457.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/1599.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/1028.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/1042.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/1123.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/1457.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/1599.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (truncated)}
\end{subfigure}%%
\caption{
    Diverse synthesized images from COCO-Body.
    We truncate the normal of SPADE and Config D, and show diverse results for Config E.
    Note that the images are randomly sampled and the latent variable for (d-g) is randomly sampled with no latent truncation.
    }
\label{fig:random_cse1}
\end{figure*}

==> tex/figures/random_cse2.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/original/1885.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/193.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/203.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/2047.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/2184.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Original}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/1885.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/193.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/203.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/2047.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/2184.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{SPADE \cite{Park_2019}}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/1885.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/193.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/203.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/2047.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/2184.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config D}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/1885.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/193.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/203.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/2047.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/2184.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/1885.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/193.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/203.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/2047.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/2184.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/1885.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/193.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/203.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/2047.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/2184.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/1885.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/193.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/203.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/2047.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/2184.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/1885.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/193.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/203.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/2047.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/2184.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{E (truncated)}
\end{subfigure}%%
\caption{
    Diverse synthesized images from COCO-Body.
    We truncate the normal of SPADE and Config D, and show diverse results for Config E.
    Note that the images are randomly sampled and the latent variable for (d-g) is randomly sampled with no latent truncation.
    }
\label{fig:random_cse2}
\end{figure*}

==> tex/figures/random_cse3.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/original/2268.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/286.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/436.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/45.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/475.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Original}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/2268.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/286.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/436.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/45.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/475.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{SPADE \cite{Park_2019}}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/2268.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/286.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/436.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/45.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/475.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config D}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/2268.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/286.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/436.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/45.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/475.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/2268.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/286.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/436.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/45.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/475.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/2268.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/286.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/436.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/45.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/475.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/2268.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/286.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/436.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/45.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/475.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/2268.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/286.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/436.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/45.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/475.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{E (truncated)}
\end{subfigure}%%
\caption{
    Diverse synthesized images from COCO-Body.
    We truncate the normal of SPADE and Config D, and show diverse results for Config E.
    Note that the images are randomly sampled and the latent variable for (d-g) is randomly sampled with no latent truncation.
    }
\label{fig:random_cse3}
\end{figure*}

==> tex/figures/random_cse4.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/original/514.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/531.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/561.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/605.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/original/925.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Original}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/514.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/531.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/561.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/605.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configB_SPADE_truncatedW/925.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{SPADE \cite{Park_2019}}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/514.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/531.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/561.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/605.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configD_truncatedW/925.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config D}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/514.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/531.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/561.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/605.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z0/925.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/514.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/531.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/561.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/605.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z1/925.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/514.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/531.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/561.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/605.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z2/925.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/514.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/531.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/561.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/605.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_z3/925.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{Config E (no truncation)}
\end{subfigure}%%
\begin{subfigure}[t]{0.122\linewidth}
\centering
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/514.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/531.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/561.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/605.png}
\includegraphics[width=\linewidth]{generated_images/random_cse/configE_truncatedW/925.png}
\captionsetup{justification=centering,textfont=small,labelfont=small}
\caption{E (truncated)}
\end{subfigure}%%
\caption{
    Diverse synthesized images from COCO-Body.
    We truncate the normal of SPADE and Config D, and show diverse results for Config E.
    Note that the images are randomly sampled and the latent variable for (d-g) is randomly sampled with no latent truncation.
    }
\label{fig:random_cse4}
\end{figure*}

==> tex/figures/truncation_experiment.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{.5\linewidth}
        \includegraphics[width=\linewidth]{figures/truncation.pdf}
        \caption{}
    \end{subfigure}%%
    \begin{subfigure}[t]{.5\linewidth}
        \includegraphics[width=\linewidth]{figures/truncation_w_interpolation.pdf}
        \caption{}
    \end{subfigure}%%
    \caption{
        Analysis of truncation techniques for \modulationMetodNoiseShort .
        \textbf{(a)} Compares different truncation strategies applied to the intermediate latent space $\omega$ or $z$. Truncation in $\omega$ yields a better trade off between diversity and image quality.
        \textbf{(b)} Evaluates the effect of $\omega$ interpolation , where we interpolate a sampled latent towards $\bar{\omega}$. Increasing the truncation (t) gradually improves image quality at the cost of sample diversity.
        }
    \label{fig:truncation_experiment}
\end{figure*}
